"Don't Step on My Toes": Resolving Editing Conflicts in Real-Time Collaboration in Computational Notebooks

Real-time collaborative editing in computational notebooks can improve the efficiency of teamwork for data scientists. However, working together through synchronous editing of notebooks introduces new challenges. Data scientists may inadvertently interfere with each others' work by altering the shared codebase and runtime state if they do not set up a social protocol for working together and monitoring their collaborators' progress. In this paper, we propose a real-time collaborative editing model for resolving conflict edits in computational notebooks that introduces three levels of edit protection to help collaborators avoid introducing errors to both the program source code and changes to the runtime state.

==> sections/05.5_additional_evaluation.tex <==
\section{Planning Session: Planning for Various Collaboration Scenarios}
\add{Noticeably, none of the participants used the cell-level access control and variable-level access control features when working with the clumsy collaborator in the paired session, although they have mentioned the potential of using these features in other collaboration setups.
To better understand the usefulness of \sys{} under various collaboration scenarios, we conducted an additional evaluation where we asked participants to plan a future collaboration session by configuring a collaborative notebook.
This additional evaluation allowed us to explore the usefulness of the \sys{} features in different collaboration scenarios. 
By asking participants to configure a collaborative notebook for planning a future collaboration session, we were able to see how they would use the collaborative features in a more proactive manner. 
This can provide valuable insights into how users might use the features of \sys{} in a variety of collaborative environments.}

\add{Overall, our additional evaluation showed that the \sys{} features can be useful in various collaboration scenarios, including working on an asynchronous paired programming session, working on tasks with high cost of error recovery, and using collaborative notebooks as lecture notes. 
By providing a way to prevent conflicts and improve organization, \sys{} can help make collaboration more efficient and effective.}
\add{\subsection{Study Setup}}
\add{In the individual study sessions, we used the same deployment as in the paired sessions. 
Based on participants' responses from the previous study, where they mentioned their prior or future use of collaborative notebooks, we synthesized three collaboration scenarios designed to be representative of various realistic situations.
For each scenario, we gave participants an initial notebook containing skeleton code and a written description of the collaboration scenario.
We asked participants to plan for the collaboration by leveraging the features of \sys{} and modifying the notebook content as necessary. 
When they finished planning, we asked participants to verbally describe their plans to the study coordinators, who would then ask a set of semi-structured interview questions to gain further insight into the participants' plans and the features they used or did not use, as well as any potential problems that might arise during the collaboration and any additional features that they felt would be useful. 
Participants were given as much time as they needed to think about their plans, with most individual sessions lasting around 30 minutes.}
\add{\subsection{Collaboration Scenarios}}
\add{In the individual session, participants were asked to plan for the following three collaboration scenarios:}
\subsubsection{Scenario 1: Asynchronous Collaboration with a Peer}
\add{For the first scenario, participants are asked to plan a paired programming session with a friend named Bob who is inexperienced with libraries like Pandas and Numpy, similar to the clumsy collaborator case in the previous study. 
However, due to conflicting schedules, Bob and the participant are unable to find a synchronous time to work together. 
This means that both of them may join and leave the session with incomplete code, and the participant cannot guarantee how Bob will use the collaborative editing features without being able to observe and intervene in Bob's actions.}
\subsubsection{Scenario 2: Working with Trainees and a High Cost of Error Recovery} 
\add{
In this scenario, we asked participants to plan a collaboration session as a full-time employee distributing tasks to interns on visualizing different aspects of the data. 
We provided participants with a notebook skeleton where the data takes a long time to load. 
In this scenario, participants needed to avoid the shared dataframe being polluted by any accidental changes, which would be costly to recover from. 
To do this, they could leverage the features of the \sys{} system to ensure that their collaboration was organized and efficient, and that the data was protected from any unintended changes.
This scenario simulates the case where error recovery could be costly in a collaboration setting. 
}
\subsubsection{Scenario 3: Classroom Sharing with Hierarchical Permissions}
\add{In this scenario, we provided participants with an educational notebook on the topic of linear regression, taken from a data science handbook. 
The first half of the notebook demonstrated the concepts, while the second half contained an exercise for students to practice what they learned.
Participants were asked to plan the use of the notebook as an instructor, taking into account the needs of the entire class during a lecture. 
They needed to ensure that they could effectively explain the concepts to the students, while also providing them with an opportunity to practice individually on the exercise. 
Additionally, the exercise included a standard solution that the instructor may want to go over with the class after they have explored their own solutions. 
Participants were asked to plan how they would like to set up the collaborative notebook at the beginning of the lecture, and how they would modify the configurations as the lecture progressed.}
\begin{table}[]
    \centering
    {\add{
    \begin{tabular}{c p{5cm} c p{4cm}}
         \toprule
        \textbf{Session} & \textbf{Action or Strategy} & \textbf{Feature} & \textbf{PID}\\
         \midrule
         Paired & Nudge the clumsy collaborator to create parallel cells & Parallel Cell & P1-14\\
         Paired & Merge parallel cells & Parallel Cell & P1, P2, P3, P5, P9, P11, P12, P14\\
         \midrule
         Planning (1) & Lock cells for loading package and data & Cell-Level Access Control & P3, P7, P10, P12, P13, P14 \\
         Planning (1) & Lock future cells & Cell-Level Access Control & P6, P10 \\
         Planning (1) & Lock the original or a copied dataframe & Variable-Level Access Control & P3, P10, P12, P13, P14 \\
         Planning (1) & Create a copy of the dataframe & --  & P3, P7, P12 \\
         Planning (1) & Ask Bob to use parallel cells & Parallel Cell & P6, P9, P13\\
         \midrule
         Planning (2) & Lock cells for loading data & Cell-Level Access Control & P3, P6, P10, P12, P13, P14 \\
         Planning (2) & Change cells' edit access so that interns can not change each others’ code & Cell-Level Access Control & P9, P12 \\
         Planning (2) & Lock the shared dataframe & Variable-Level Access Control & P3, P6, P7, P10, P12, P13, P14 \\
         Planning (2) & Ask the interns to use the parallel cells 
         & Parallel Cell & P3, P6, P9\\
         Planning (2) & Create a copy of the dataframe if needed & -- & P7, P10 \\
         \midrule
         Planning (3) & Lock editing access for code cells in lecture notes & Cell-Level Access Control & P3, P6, P7, P9, P10, P12, P13, P14 \\
         Planning (3) & Lock reading access for code cells in lecture notes that are not covered yet & Cell-Level Access Control & P6, P10 \\
         Planning (3) & Lock reading access for the standard solution code cell in the exercise & Cell-Level Access Control &  P3, P6, P9, P10, P12, P14\\
         Planning (3) & Lock access for variables generated in lecture notes & Variable-Level Access Control & P13\\
         Planning (3) & Lock access for the variable for storing results in the exercise & Variable-Level Access Control & P14 \\
         Planning (3) & Create parallel cells for students to work on the exercise & Parallel Cell & P3, P7, P9, P10, P12, P13, P14 \\
         Planning (3) & Ask students to use parallel cells if they want to explore the code (e.g., change parameters) in lecture notes & Parallel Cell & P9, P12 \\
         \midrule
         Group & Create parallel cells & Parallel Cell & P3, P4, P7, P9, P10, P14 \\
         Group & Merge parallel cells & Parallel Cell & P4, P7, P9 \\
         Group & Sync parallel cells & Parallel Cell & P3 \\
         \bottomrule
    \end{tabular}
    }}
    \caption{\add{Features that participants have used for tasks in each study.}}
    \label{tab:strategy}
\end{table}

\add{\subsection{Data Analysis}}
\add{In each of the above scenarios, participants were asked to configure a shared notebook.
We used three metrics to understand and evaluate the effectiveness of the participants' specified notebook configurations.
% We collected three data sources to understand the effectiveness of the configuration. 
First, we summarize the patterns in how participants set up collaborative notebooks for each scenario. 
% Second, we identified and form lists of potential editing conflicts that might occur in each scenario.
The second data source was a list of potential editing conflicts that may occur in each scenario, which was identified by the research team. 
We used this list to test participants' configurations against the potential conflicts and analyze their reliability in addressing them. 
Lastly, we recorded and transcribed participants' post-task reflections, in which they discussed their choices, potential problems, and suggestions for additional features. 
These data sources gave us a comprehensive view of the effectiveness of the configuration in different collaboration scenarios.}
\add{\subsection{Results}}
\subsubsection{Usage of the Collaborative Features for Each Scenario}
\add{
In Table \ref{tab:strategy}, we summarize the strategies that participants described for each scenario and listed the features of \sys{} that are involved.
For the first scenario of working in an asynchronous paired programming session, three participants chose to ask the collaborator to use the parallel cells for exploration, while the other participants chose to use cell-level or variable-level access controls.
P12 explained why their strategy changed compared to the clumsy collaborator scenario in the previous paired session:
\begin{quote}
    I can't really trust that Bob is going to use parallel cells because we are not working together at the same time. I want to set up everything for him so he can only access the things he need.
\end{quote}}

\add{For the second scenario, most participants except P10 chose to lock the shared variable to prevent it from being polluted. 
Participants suggested that the interns could use parallel cells or make a copy of the dataframe if needed.
In addition, most participants (6 out of 8) chose to restrict the editing access of the code cell for loading the data, while two of them also chose to set up the editing access for the code cells that are assigned to each individual intern.}

\add{In the last scenario, participants described a mixed strategy for planning the collaborative notebook for a data science classroom.
All participants decided to turn off the editing access for code cells in lecture notes, as P14 explained:
\begin{quote}
    I would turn off the cell editing for the class. Otherwise, if there's so many students, it is easy for someone to accidentally hit a backspace somewhere or something and mess things up.
\end{quote}
Some participants (P9 and P12) mentioned that they would create a copy of the cell below each code cell for lecture notes and make them into parallel cells, in case students want to explore the code cells in lecture notes.
For the same consideration, P13 wanted to restrict the access for variables generated in lecture notes, in case students modify the shared runtime in lecture.
Other participants did not worry about protecting the shared variables, as one participant explained (P6):
\begin{quote}
    Since the content of the code cell is locked, I can always restart the kernel and run the notebook from the beginning if anything goes wrong.
\end{quote}
In addition, two participants (P6 and P10) mentioned that they would like to change the code cells' reading access as the lecture progresses so that students can stay focused.
For the exercise part, most participants planned to hide the reference solution code (6 out of 8) and ask students to work on parallel cells for their own practice (7 out of 8).}

\begin{table}[]
    \centering
    {\add{
    \begin{tabular}{c p{10cm} c c}
        \toprule
        \textbf{Scenario} & \textbf{Editing Conflicts} & \textbf{Category} & \textbf{Pass Rate}  \\
        \midrule
        Scenario 1 & Bob dropped all the NA values in the dataset. & Common & 0.75 \\
        Scenario 1 & Bob changed the importing package cell to only include a subset of a package. & Common & 0.75 \\
        Scenario 1 & Bob missed the instruction and started to work on the last code cell. & Rare & 0.25 \\
        \midrule
        Scenario 2 & Intern A changed the shared dataframe. & Common & 0.88 \\
        Scenario 2 & Intern A run the code cell for loading the data frame. & Common & 0.88 \\
        Scenario 2 & Intern A and intern B have the same naming of a variable. & Rare & 0.38 \\
        \midrule
        Scenario 3 & A student edited the code cells for demonstration. & Common & 1 \\
        Scenario 3 & Students directly assigned the prediction results to the shared data frame. & Common & 0.88 \\
        Scenario 3 & Students executed a code cell multiple times. & Rare & 0.13 \\
        \bottomrule
    \end{tabular}
    }}
    \caption{\add{For each scenario, the research team solicited three potential cases for editing conflicts and run through participants' notebooks through these cases.}}
    \label{tab:rubric}
\end{table}
\subsubsection{Effectiveness of the Collaboration Plan}
\add{For each scenario, we solicited three potential conflicts that may arise during collaboration: two that we expect to be common and one that is less likely to occur. 
We then evaluated each participant's use of the collaborative notebook to determine if their configuration could effectively address these conflicts. 
Two members of the research team carefully calibrated and discussed the ratings until they reached a consensus. 
The results, shown in Table \ref{tab:rubric}, indicate that most participants (more than 6 out of 8) were able to utilize the features in \sys{} to successfully address common collaboration issues. 
Even for the less likely problems (e.g., Bob missing the instruction and starting work on the last code cell in the first scenario), a small number of participants (1--3) were still able to successfully handle these rare cases.}
\subsubsection{Improving Access Control}
\add{In the reflective interview, participants mentioned several potential problems and suggested improvements for the collaboration scenarios in the current system design.}

\add{First, participants brought up the need for better access control on the notebook level. For example, P13 mentioned that restarting or interrupting the notebook kernel in the third collaboration scenario could cause problems when the instructor is demonstrating concepts. Other types of access control mentioned by participants included preventing collaborators from executing a code cell (P6) or copying and pasting the content from a code cell (P13).}

\add{Participants also suggested ways to improve the process of configuring access control. 
For example, in the first scenario, P6 and P10 mentioned that they would like to restrict cell edit access for their collaborator for every new code cell that they create under a section.
One participant also suggested adding a ``run and lock all cells and variables above'' button (P13) to avoid the need to manually lock all code cells in the lecture notes in the third scenario.}

\add{Lastly, participants (P9 and P12) mentioned the potential benefits of combining cell access control with parallel cells. This would be particularly useful in the third scenario, where the instructor may not want students to see each other's solutions in the parallel cell.}

==> sections/06_evaluation_group.tex <==
\section{Group Session: Case Study on Open-Ended Collaboration}
\add{The paired session and the individual session demonstrated the usefulness of \sys{} in designated collaboration setups. 
To further understand how \sys{} would be used in open-ended and less-structured collaboration tasks, we conducted two case studies by observing participants as they worked together in groups on a collaborative task.}

\add{Overall, our case studies showed that \sys{} can be useful in open-ended and less-structured collaboration tasks. 
By providing a framework for organizing the collaboration, it can help them divide up the work and ensure that each person is working on a specific part of the task. This can help make the collaboration more efficient and reduce the risk of overlap or duplication of effort.
Additionally, \sys{} can help prevent conflicts between collaborators, save time and reduce frustration, leading to a more productive collaboration.}

\subsection{Study Setup}

The group study sessions were also conducted remotely, and used the same deployment as the individual sessions.
In the group sessions, participants communicated by talking to each other through the video-conferencing application.

As all participants had already used the extension in individual sessions, we started with a brief reminder about its features.
Then, one researcher would explain the collaborative task to the participants, and ask participants to introduce themselves to their collaborators.
Next, we explained the open-ended tasks and dataset.
In the first group (4 participants), we assigned the participant who is most experienced in data science as the team leader to mitigate collaboration during the task.
We did not assign a group leader in group two, which only had 3 participants.
Each session lasted 60 minutes in total, and participants were given 40 minutes to complete the task.
We would remind the participants to clean up the notebook to provide final results when there were 5 minutes left.
Finally, we asked each participant to fill out a post-task survey regarding their collaboration experience.

\subsection{Task Description}
In the group task, participants were asked to conduct an exploratory analysis of papers accepted by CHI 2022.
We provided the participants with two datasets: the first one contains the paper name, link, and author list of full papers; the second one contains the name, link, and affiliations of authors.
To make the task more authentic, we collected the raw data by scraping the actual conference program from \add{2022}.
Participants were given a list of open-ended tasks regarding ranking authors and institutions by the number of full papers they published.
To complete the task, they would need to conduct a series of data pre-processing and cross-referencing between two datasets, and the process is highly open-ended. 
For example, the format for authors' names in two datasets are different; authors from different institutions might have the same name; an author may have multiple institutions; or even the name of the same institution can be put differently in the system.
We made participants aware of the complication in the dataset, but did not provide detailed instructions to encourage open-ended exploration.
% \begin{itemize}
%     \item We asked participants to conduct 
%     \item To make the task more authentic, we collect the raw data by scraping last years' program
%     \item we are interested in author rank, institution rank
%     \item 
%     \item we did not provide detailed instructions, make it open-ended;
% \end{itemize}

\add{\subsection{Data Analysis}}
\add{During each group session, two members of the research team closely monitored collaboration activities and took detailed observational notes. 
We also recorded participants' screens and captured key activity logs from the Jupyter Notebook to help us understand the collaborative workflow of each group. 
In addition, we conducted a second pass on the video recordings to identify instances of collaboration challenges and undesired behaviors. 
This allowed us to carefully analyze the collaboration process and identify areas for improvement.}

\subsection{Result}
Overall, we observed different collaboration patterns among the two groups.
We report how the two groups leveraged \sys{} to support their workflow.
\begin{figure*}
\includegraphics[width=\textwidth]{figures/group_viz.pdf}
  \caption{The collaborative workflow for G1 and G2.}
  \label{fig:group1_workflow}
\end{figure*}
\subsubsection{G1: Starting from Pair Authoring}
We observed that participants in G1 used a mixed of collaboration styles, including pair authoring, divide and conquer, and competitive authoring.
With a group leader moderating the discussions, the team naturally started the task by a pair authoring mode.
Figure \ref{fig:group1_workflow} illustrates the collaborative workflow of G1. 
We broke down their exploration process into four stages.

\begin{itemize}
    \item \textbf{Stage 1:} To begin with, the four participants (P4, P7, P10, P12) discussed the task and decided to split paper authors first. Then, P4 proposed to begin work and they used a pair authoring mode where P4 directly wrote code in the notebook. The rest of the team closely watched him coding and helped him with debugging.
    \item \textbf{Stage 2:} Next, the team leader P12 proposed two tasks -- lower casing the authors' names and summarizing authors' paper counts. The team then split into two groups where P10 worked on lower casing, P4 and P7 worked on summarizing the counts, and P12 observed the process. P10 quickly implemented lower casing by directly working on the code cell while the rest of the team is still discussing how to summarize the counts. P10 then turned on the cell editing lock to her finished code cells. In the meanwhile, P4 and P7 created two parallel cell groups and started to work on summarizing the counts in competitive authoring style. After P4 figured out the correct solution, he reported to P12 and they decided to merge his solution into the main notebook. However, noticing that P7 was still working on his solution, P4 chose to mark his cell group as the main version in the parallel groups and moved on to the next task with P12.
    \item \textbf{Stage 3:} Moving on to the next stage, P4, P10, and P12 started to examine the author---affiliations table using parallel cell groups. Then, P7 finished his implementation of summarizing author counts and reported to the team. P7 proposed to unindent the parallel cell group to keep P4's solution. After they merged the cells for summarizing authors count, P7 proposed to branch off and work on creating a histogram visualization of the authors' paper count while the rest of the team kept exploring the author---affiliations table. After P7 finished the histogram visualization in a parallel cell, he notified the rest of the team and merged his exploration code.
    \item \textbf{Stage 4:} Lastly, all the team members worked together on merging duplicates in institution names since they realized that there \add{was not much time left}. They created a parallel cell group with four tabs where everyone worked on their own tab. They were not able to finish this task towards the end of the study.
\end{itemize}

\subsubsection{G2: Starting from Divide and Conquer}
G2 started with the divide and conquer style where the three members decided to work on three different tasks --- authors' paper count, institutions' paper count, and institutions' paper count without duplicates.
The team also discussed and agreed on using parallel cell groups whenever they started to work, and merging them to the main notebook after they verified the results.
P3 proposed to lock the shared variables as well.
The team decided to stick with the protocol of using parallel cell groups because they agreed that \say{If we are all working in indented cells, we don't need to lock the dataframes} (P3).
We broke down their exploration process into three stages:
\begin{itemize}
    \item \textbf{Stage 1}: The three participants started by indenting three cells and working individually on the three tasks. However, the tasks for P3 and P9 both required splitting institution lists. P3 and P9 took two different approaches for the splitting, where P3 splitting the institutions into columns and P9 splitting the institutions into rows. P9 realized it and started a discussion with P3. In the meanwhile, P14 was working individually on splitting the list of authors for each paper.
    \item \textbf{Stage 2}: In this stage, P3 and P9 turned into pair authoring mode after realizing that their tasks need the same pre-processing. After the discussion, P3 was convinced to split the institution list into rows and she attempted to do it in her previous cell. After she finished, she continued to discuss with P9 and observed P9 coding. P9 first attempted to count institutions' papers.
    After realizing the need to cross reference two tables, P9 and P3 turned to work on formatting authors' name in the author--affiliations table.
    At this stage, P9 did most of the programming and P3 actively participated in discussions.
    On the other hand, P14 continued to work individually on counting authors' paper numbers.
    \item \textbf{Stage 3}: In this stage, P3 and P9 decided to both try to create a cross-reference between the two tables. P3 asked P9 to merge his previous code into the main notebook, and performed a sync to update her parallel cell group. Then, they began to work competitively on cross reference.
    Meanwhile, P14 continued to work individually on creating a histogram visualization of the authors' papers.
\end{itemize}

\subsubsection{Reflections on the Collaborative Session}
By observing two groups attempting the task with different collaboration strategies, we found that \sys{} was stable and effective in preventing conflict edits while being flexible to support various ad-hoc combinations of collaboration models.
We did not observe instances of the abused copying of data frames.
We also did not observe instances where participants messed up with the shared notebook and needed to restart the kernel.
In the reflection questionnaire, participants commented that \say{it's a very nice tool for collaboration} (P7); \say{it helps a lot when we are exploring the dataset and trying to test some functions.} (P10).
In particular, P9 mentioned:
\begin{quote}
    This tool is very helpful. It allows us to split the tasks amongst the team, work independently without having to worry about interference, but still be able to discuss problems with each other's solutions if needed.
\end{quote}

In addition, participants also reported things that did not work well in the collaboration session.
For example, P14 in G2 who spent most of the session working independently on the authors' paper count complained that the pre-processing approach in her task (e.g., split author list) is similar to her collaborators' tasks (e.g., split institution list). 
But they did not collaboratively work on the pre-processing:
\begin{quote}
    It helped us avoid running cell blocks that would influence each other's work and allowed us to work on our own parts. However, it also made us communicate less and made us focus on our own parts when a lot of the questions could've been solved with the majority of the data cleaning work being the same.
\end{quote}

==> sections/09_ack.tex <==
  \begin{acks}
  test
  \end{acks}
